Toward Realistic Solar Flare Models: An explicit Particle-In-Cell solver in the DISPATCH framework

Context. Simulating solar flares, which involve large-scale dynamics and small-scale magnetic reconnection, poses significant computational challenges. Aims. This study aims to develop an explicit Particle-In-Cell (PIC) solver within the DISPATCH framework to model the small-scale kinetic processes in solar corona setting. This study in the first in a series with the ultimate goal to develop a hybrid PIC-MHD solver, to simulate solar flares. Methods. The PIC solver, inspired by the PhotonPlasma code, solves the Vlasov-Maxwell equations in a collisionless regime using explicit time-staggering and spatial-staggering techniques. Validation included unit tests, plasma frequency recovery, two-stream instability, and current sheet dynamics. Results. Validation tests confirmed the solver's accuracy and robustness in modeling plasma dynamics and electromagnetic fields. Conclusions. The integration of the explicit PIC solver into the DISPATCH framework is the first step towards bridging the gap between large and small scale dynamics, providing a robust platform for future solar physics research.

==> Sections/Performance.tex <==
\section{Performance}
\textcolor{red}{Maybe we don't need this in this article}
